Observation of Energetic Jet Production in pp Collisions at sqrt(s) = 7 TeV using the ATLAS Experiment at the LHC

We report the observation of energetic jet production in proton-proton collisions at sqrt(s) = 7 TeV, based on about 1 nb^-1 of integrated luminosity collected by the ATLAS detector. The anti-kT algorithm is used to reconstruct jets with pT > 30 GeV and |y| < 2.8. Jets with pT up to ~500 GeV and events with dijet mass up to ~1 TeV are observed. The jet shapes and charged particle flow confirm that the observed jet signal corresponds to collimated flows of particles in the final state.

==> Makefile <==
######################################################################
# LaTeX Makefile
# $Id$
######################################################################

PROJECT = Feng_Eric
LATEX = latex
STYLEFILES = *.sty

all: pdf

pdf: $(PROJECT).pdf

$(PROJECT).pdf: $(PROJECT).tex *.tex
	latex $(PROJECT).tex && latex $(PROJECT).tex && dvips $(PROJECT).dvi && ps2pdf $(PROJECT).ps

clean:
	rm -f $(PROJECT).dvi $(PROJECT).log \
	      $(PROJECT).aux $(PROJECT).blg $(PROJECT).toc \
	      $(PROJECT).bbl $(PROJECT).out \
	      missfont.log symbols.aux ordercite

